Relevance Vector Machines for harmonization of MRI brain volumes using image descriptors

With the increased need for multi-center magnetic resonance imaging studies, problems arise related to differences in hardware and software between centers. Namely, current algorithms for brain volume quantification are unreliable for the longitudinal assessment of volume changes in this type of setting. Currently most methods attempt to decrease this issue by regressing the scanner- and/or center-effects from the original data. In this work, we explore a novel approach to harmonize brain volume measurements by using only image descriptors. First, we explore the relationships between volumes and image descriptors. Then, we train a Relevance Vector Machine (RVM) model over a large multi-site dataset of healthy subjects to perform volume harmonization. Finally, we validate the method over two different datasets: i) a subset of unseen healthy controls; and ii) a test-retest dataset of multiple sclerosis (MS) patients. The method decreases scanner and center variability while preserving measurements that did not require correction in MS patient data. We show that image descriptors can be used as input to a machine learning algorithm to improve the reliability of longitudinal volumetric studies.

==> old_text.tex <==
%, which results in very \emph{sparse} inferred predictors. 
%  governed by a set of hyperparamenters, one associated with each weight
% ,




% if we consider a dataset of real-valued input-target pairs $\{x_n, t_n\}_{n=1}^{N}$, the model defines a conditional distribution of the type: 
% $p(t_n|x) = \mathcal{N}(t_n|y(x_n), \beta^-1),$ 
% which specifies a Gaussian distribution over $t_n$ with mean $y(x_n)$ and variance $ \beta \equiv \sigma^{-2}$ (for convenience). The mean is given by a linear model of the form:
% $ y(\mathbf{x}) = \sum_{i=1}^{N}w_i K(\mathbf{x, x_i}) + w_0 ,$ where $K(\mathbf{x},\mathbf{x_i}) \equiv \phi(\mathbf{x})$ is a kernel parametrised by the training vectors defining a basis function. 
% % In contrast to SVM there is no restriction to positive definite kernels.

% To avoid over-fitting due to a large number of parameters, a zero-mean Gaussian prior probability distribution is defined over the parameters: 

% $
%     \qquad p(\mathbf{w}|\mathbf{\alpha}) = \prod_{i=0}^{N} \mathcal{N}(w_i|0, \alpha_i^{-1}),
% $
% % $p(\mathbf{w}|\mathbf{\alpha}) = \prod_{i=0}^{N} \mathcal{N}(w_i|0, \alpha_i^{-1}),$
% where $\mathbf{\alpha}$ is the precision of the corresponding parameter $\mathbf{w}$. 

% The posterior distribution for the weights is again Gaussian and takes the form:
% $p(\mathbf{w}|\mathbf{t},\mathbf{\alpha}, \beta) =  \mathcal{N}(\mathbf{w}|\mathbf{\mu},\Sigma), $
% where the posterior covariance and mean are:
% \[
% \Sigma = (\beta \Phi^{T}\Phi+A)^{-1},  \qquad \mu = \beta \Sigma \Phi^Tt, 
% \]
% where $A = diag(\alpha_0, \alpha_1,...,\alpha_N)$

% Thus, relevance vector learning is the search for the hyperparameter posterior with respect to $\alpha$ and $\beta$ that maximizes the term $p(t|\alpha,\beta)$ (the marginal likelihood, or evidence):
% \[ \ln p(t|\alpha, \sigma^2) = -\frac{1}{2}{N \ln(2\pi)+\ln|C|+t^TC^{-1}t} \quad 
% \textrm{with} \quad C = \beta^{-1}I+\Phi A^{-1}\Phi^T \]
% The learning algorithm proceeds by iteratively updating $\alpha$ and $\beta$:

% \[
% \alpha_{i}^{new} = \frac{\gamma_i}{\mu_i^2} \ \textrm{with} \ 
% \gamma_i \equiv 1-\alpha_i\sigma_{ii}, \quad 
% (\beta^{new})^{-1} = \frac{\|t-\Phi\mu\|^2}{N-\sum_i\gamma_i}
% \]

% In practice, during re-estimation, many $\alpha$ tend to infinity, which implies that the posterior distributions of many of the weights peak around zero. The basis functions associated with these parameters do not influence the predictions and can be pruned out, which results in a sparse model.  The remaining non-zero weights are called \emph{relevance} vectors, and can be seen as analogous to the \emph{support vectors} in a support vector machine. 

% Finally, we can make predictions for new data points using $y_* = \mu^T \phi(\mathbf{x_*})$.
% % When we maximize the evidence with respect to these hyperparameters, a significant portion of them go to infinity, and the corresponding weight parameters have posterior distributions that are concentrated at zero. The basis functions associated with these parameters thereforte play no role in the predictions made by the model and so are pruned out, resulting in a sparse model. 

% %  which is achieved because the posterior distributions of many of the weights peak around zero. The remaining non-zero weights are termed \emph{relevance} vectors - analogous to the \emph{support vectors} in a SVM. This formulation of prior distributions is a mechanism of \emph{automatic relevance determination} \cite{MacKay1992}.
% % Relevance vector learning involves the maximization of the product of the marginal likelihood and the priors over $\alpha$ and $\sigma^2$ (or $\beta \equiv \sigma^2 $ for convenience. 

% % Expectation-Maximization Updates:
% % considering scalar-valued target functions only, we follow the standard probabilistic formulation and assume that the targets are samples from the model with additive noise:
% % $t_n=y(x_n;\textbf{w})+\epsilon_n$,  
% % where $\epsilon_n$ are independent samples from some noise process which is further assumed to be mean-zero Gaussian with variance $\sigma^2$. Thus, the model defines a conditional distribution of the form: $p(t_n|x) = \mathcal{N}(t_n|y(x_n), \sigma^2)$
% % which specifies a Gaussian distribution over $t_n$ with mean $y(x_n)$ and variance $\sigma^2$.


% % Having defined the prior, Bayesian inference proceeds by computing the posterior over all unknowns in the given data:

% % $ p(w,\alpha, \sigma^2 |t) = \frac{p(t|w,\alpha, \sigma^2) p(w,\alpha, \sigma^2)}{p(t)} $


% \newpage
